The First Pathloss Radio Map Prediction Challenge

To foster research and facilitate fair comparisons among recently proposed pathloss radio map prediction methods, we have launched the ICASSP 2023 First Pathloss Radio Map Prediction Challenge. In this short overview paper, we briefly describe the pathloss prediction problem, the provided datasets, the challenge task and the challenge evaluation methodology. Finally, we present the results of the challenge.

==> header.tex <==
%\documentclass[journal]{IEEEtran}
%\documentclass[11pt,draftclsnofoot,peerreviewca,letterpaper,onecolumn]{IEEEtran}

\usepackage{amsfonts, amscd, mathrsfs, amsopn, bbm, bbold, multicol, relsize}
\usepackage{mathrsfs}
\usepackage[psamsfonts]{amssymb}
\usepackage{mathbbol}
\usepackage[mathscr]{eucal}
\usepackage[cmex10]{amsmath}
\usepackage[amsmath,thmmarks]{ntheorem}
\usepackage{mathtools}
%\usepackage{subfigure}
%\usepackage{caption}
%\usepackage{subcaption}
\usepackage{cite}
\usepackage{tikz}
\usepackage{graphicx}
%\graphicspath{{../pdf/}{../jpeg/}}
%\DeclareGraphicsExtensions{.pdf,.jpeg,.png}
%\interdisplaylinepenalty=2500
%\usepackage{array}
%\usepackage[caption=false,font=footnotesize]{subfig}

% ---------- Theorems ----------
\theorempreskipamount0.618ex
\theorempostskipamount0.618ex

\theoremstyle{plain}
\theoremheaderfont{\itshape\bfseries}
\theorembodyfont{\normalfont\itshape}
\theoremseparator{:}
\theoremsymbol{}%\vspace{0.2cm}}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{problem}{Problem}
\newtheorem{definition}{Definition}
\newtheorem{claim}{Claim}
\newtheorem{remark}{Remark}
\newtheorem*{algo}{Algebraic Reconstruction Algorithm}

\theoremstyle{nonumberplain}
\newtheorem{defi}{Definition}
\newtheorem{cond}{Condition~G}

\theoremstyle{nonumberplain}
\theoremheaderfont{\itshape}
\theorembodyfont{\normalfont}
\theoremseparator{:}
\theoremsymbol{}


\theoremstyle{plain}
\theoremheaderfont{\itshape\bfseries}
\theorembodyfont{\normalfont}
\theoremseparator{:}
\newtheorem{example}{Example}

\theoremstyle{nonumberplain}
\theoremsymbol{\rule{1ex}{1ex}}
\newtheorem{proofsketch}{Sketch of proof}
\newtheorem{proof}{Proof}
% -------------------------------
\newlength\fheight
\newlength\fwidth
\setlength\fheight{4cm}
\setlength\fwidth{6cm}

% ----- Definitions -----

\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\DeclarePairedDelimiter\inn{\langle}{\rangle}
\DeclarePairedDelimiter\lrbrace{\lbrace}{\rbrace}
\DeclarePairedDelimiter\gausskl{\left\lceil }{\right\rceil}


\def\aut{\text{Aut}}
\def\hom{\text{Hom}}
\def\map{\text{Map}}

\def\pr{\text{pr}}



\def\X{\mathcal{X}}

\def\Alg{\mathfrak{A}}
\def\Bor{\mathfrak{B}}
\def\Gen{\mathfrak{G}}
\def\cqua{\mathfrak{I}}
\def\Leb{\mathfrak{L}}
\def\nul{\mathfrak{N}}


\def\d{ \mathrm{d} }								% integral d
\def\I{ \mathrm{i} }								% imaginary unit
\def\E{ \mathrm{e} }								% e
\def\T{ \mathrm{T} }								% T - transpose
\def\Em{\mathrm{E}}
\def\Gm{\mathrm{G}}
\def\Hm{\mathrm{H}}
\def\Op{\mathrm{O}}
\def\Um{\mathrm{U}}
\def\Vm{\mathrm{V}}
\def\Wm{\mathrm{W}}
\def\Analy{\mathrm{C}}
\def\Synth{\mathrm{R}}
\def\Frame{\mathrm{S}}
\def\Ann{\mathrm{A}}
\def\Compo{\mathrm{U}}


\def\nat{ \mathbb{N} }								% set of natural numbers
\def\Ber{ \mathbb{B} }	
\def\Bert{ \tilde{\Ber} }
\def\Der{\tilde{D}}
\def\Lambt{\tilde{\Lambda}}
\def\natz{ \nat_{0} }                 % set of natural numbers included 0
\def\inte{ \mathbb{Z} }								% set of whole numbers
\def\inten{\mathbb{Z}^{N}}
\def\comp{ \mathbb{C} }								% complex numbers
\def\real{ \mathbb{R} }								% real numbers
\def\realn{\mathbb{R}^{N}}
\def\field{ \mathbb{F} }
\def\rat{ \mathbb{Q} }


\def\CN{ \comp }	
\def\RN{ \real }
\def\Hx{ \widehat{x} }
\def\Hy{ \widehat{y} }
\def\TT{ \mathbb{T} }                             	% subset of R

\def\uD{ \mathbb{D} }								% unit disk
\def\uC{ \mathbb{T} }								% unit circle
\def\uDD{ \overline{\mathbb{D}} }   % closed unit disk

%\def\A{ \mathcal{A} }
\def\B{ \mathcal{B} }								% Banach space 
\def\D{ \mathcal{D} }
\def\G{ \mathcal{G} }
\def\H{ \mathcal{H} }								% Hilbert space 
\def\Ical{\mathcal{I}}
\def\J{\mathcal{J}}
\def\K{ \mathcal{K} }								% Hilbert space
\def\Leb{ \mathcal{L} }		
\def\N{ \mathcal{N} }								
\def\S{ \mathcal{S} }               % Subspace S
%\def\V{\mathcal{V}}
\def\W{\mathcal{W}}
\def\O{\mathcal{O}}
%\def\P{\mathcal{P}}
\def\Ti{\mathcal{T}}
\def\X{\mathcal{X}}
%\def\Y{\mathcal{Y}}
\def\PW{\mathcal{PW}}
\def\Ex{\mathcal{E}}

\def\funcb{\mathbf{f}}
\def\funcbt{\tilde{\mathbf{f}}}
\def\eb{\mathbf{e}}
\def\ab{\mathbf{a}}
\def\vpb{\pmb{\phi}}
\def\varpb{\pmb{\varphi}}
\def\nub{\boldsymbol{\nu}}


\def\CT{ \mathcal{C}(\uC)}					% Continuous Functions on Unit Circle
\def\Hol{\text{Hol}}

% ----- Subspaces ------
\def\Do{ \mathscr{D} }								% Domain
\def\Ra{ \mathscr{R} }								% Range
\def\Nu{ \mathscr{N} }								% Null space

% ----- bold characters - vectors -----
\def\be{ \mathbf{e} }									% bold e
\def\bs{ \mathbf{s} }									% bold s
\def\bx{ \mathbf{x} }									% bold x
\def\by{ \mathbf{y} }									% bold y

% ---------- Matrizen ----------
\def\bA{ \mathbf{A} } 								% bold A
\def\bB{ \mathbf{B} } 								% bold B
\def\bC{ \mathbf{C} } 								% bold C

\def\bPhi{ \boldsymbol\varPhi }				% bold Phi
\def\bLambda{ \boldsymbol\Lambda }		% bold Lambda

% ----- boldsymbols - sequences -----
\def\bsc{ \boldsymbol{c} }						% boldsymbol c
\def\bse{ \boldsymbol{e} }						% boldsymbol e
\def\bsf{ \boldsymbol{f} }						% boldsymbol f
\def\bss{ \boldsymbol{s} }						% boldsymbol s
\def\bsw{ \boldsymbol{w} }						% boldsymbol w
\def\bsx{ \boldsymbol{x} }						% boldsymbol x
\def\bsy{ \boldsymbol{y} }						% boldsymbol y
\def\bssigma{ \boldsymbol{\sigma} }		% boldsymbol sigma
\def\bsvarphi{ \boldsymbol{\varphi} }	% boldsymbol phi
\def\bmu{ \boldsymbol{\mu} }	% boldsymbol phi

\def\varphik{\varphi_{k}}    %varphi _{k}
\def\varphikint{\left\{ \varphik \right\} _{k\in\inte}} %varphi_{k element int}

% --- Spezielle Operatorensymbole -----
\def\FT{ \mathcal{F} }										% Fourier transform
%\def\U{ \mathrm{U} }											% an unitary operator
\def\Tr{ \mathrm{T} }											% translation operator
\def\Mo{ \mathrm{M} }											% modulation operator
\def\Di{ \mathrm{D} }											% dilatation operator
\def\Sy{ \mathrm{S} }           %synthesis operator
\def\Pr{ \mathrm{P} }
\def\Fr{\mathrm{F}}
\def\Hf{\mathrm{H}}
\def\quo{\mathrm{q}}


\newcommand{\Tsf}{{\sf T}}

% ------------------------
%Lebesgue r�ume
\def\ltwointe{l^{2}({\inte})}
\def\Ltworeal{L^{2}({\real})}
\def\Lonereal{L^{1}({\real})}
\def\LoneuC{L^{1}({\uC})}
\def\LtwouC{L^{2}({\uC})}


\def\akint{\left\{a_{k}\right\}_{k\in\inte}}
\def\ckint{\left\{c_{k}\right\}_{k\in\inte}}
\def\dkint{\left\{d_{k}\right\}_{k\in\inte}}
\def\ekint{\left\{e_{k}\right\}_{k\in\inte}}
\def\fkint{\left\{f_{k}\right\}_{k\in\inte}}
\def\gkint{\left\{g_{k}\right\}_{k\in\inte}}
\def\skint{\left\{s_{k}\right\}_{k\in\inte}}
\def\wkint{\left\{w_{k}\right\}_{k\in\inte}}



\def\R{\mathcal{R}}
\def\N{\mathcal{N}}
%\def\A{\mathcal{A}}
\def\M{\mathcal{M}}

\DeclareMathOperator*{\argmin}{\text{argmin}}
\DeclareMathOperator{\maxx}{\text{max}}
%\DeclareMathOperator{\min}{min}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\spark}{\text{spark}}
\def\krank{\sigma}
\newcommand{\A}{{\bf A}}
\newcommand{\V}{{\bf V}}
\newcommand{\U}{{\bf U}}
\newcommand{\Q}{{\bf Q}}
\def\P{{\bf P}}
\newcommand{\F}{{\bf F}}
\newcommand{\mF}{{\mathcal{F}}}
\def\mFz{\mF_0}
\newcommand{\fnyq}{{f_\textrm{NYQ}}}
\newcommand{\mM}{{\mathcal{M}}}
\def\tx{{\tilde{x}}}
\newcommand{\y}{{\bf y}}
\newcommand{\Y}{{\bf Y}}
\newcommand{\x}{{\bf x}}
\newcommand{\z}{{\bf z}}
\newcommand{\cn}{{\bf c}}
\newcommand{\Z}{{\bf Z}}
\def\yn{\y[n]}
\def\zn{\z[n]}
\def\cnn{\cn[n]}
\newcommand{\eg}{{\em e.g., }}
\newcommand{\ie}{{\em i.e., }}
\newcommand{\expp}[1]{e^{#1}}
\def\balpha{ \boldsymbol{\alpha} }

\DeclareMathOperator{\ess}{\text{ess}}
\DeclareMathOperator{\supp}{\text{supp}}
\DeclareMathOperator{\spn}{\text{span}}
\DeclareMathOperator{\sinc}{\text{sinc}}
\DeclareMathOperator{\ran}{\text{ran}}
\DeclareMathOperator{\id}{\text{Id}}
\DeclareMathOperator{\re}{\text{Re}}
\DeclareMathOperator{\ima}{\text{Im}}
\DeclareMathOperator{\dom}{\text{Dom}}
\DeclareMathOperator{\inc}{\text{inc}}
\DeclareMathOperator{\snr}{\text{SNR}}
\DeclareMathOperator{\sgn}{\text{sgn}}
\DeclareMathOperator{\argo}{\text{arg}}
%\DeclareMathOperator{\Im}{\text{Im}}
%\DeclareMathOperator{\Re}{\text{Re}}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\essinf}{ess\,inf}
\DeclareMathOperator*{\suchthat}{s.t.}
\DeclareMathOperator*{\trace}{trace}
\DeclareMathOperator*{\Trace}{\text{tr}}
\newcommand{\HS}{\text{HS}}
\def\eps{ \epsilon }
\def\phieps{ \phi_{\epsilon} }
\def\bX{ \mathbf{X} }
\newcommand{\Opp}[1]{\mathrm{#1}}
\DeclareMathOperator*{\rank}{rank}

\newcommand{\HR}[1]{{{#1}}}
%\DeclareMathOperator{\ker}{\text{ker}}

\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  %\vphantom{\big|} % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}


